Coordinating Followers to Reach Better Equilibria: End-to-End Gradient Descent for Stackelberg Games

A growing body of work in game theory extends the traditional Stackelberg game to settings with one leader and multiple followers who play a Nash equilibrium. Standard approaches for computing equilibria in these games reformulate the followers' best response as constraints in the leader's optimization problem. These reformulation approaches can sometimes be effective, but often get trapped in low-quality solutions when followers' objectives are non-linear or non-quadratic. Moreover, these approaches assume a unique equilibrium or a specific equilibrium concept, e.g., optimistic or pessimistic, which is a limiting assumption in many situations. To overcome these limitations, we propose a stochastic gradient descent--based approach, where the leader's strategy is updated by differentiating through the followers' best responses. We frame the leader's optimization as a learning problem against followers' equilibrium, which allows us to decouple the followers' equilibrium constraints from the leader's problem. This approach also addresses cases with multiple equilibria and arbitrary equilibrium selection procedures by back-propagating through a sampled Nash equilibrium. To this end, this paper introduces a novel concept called equilibrium flow to formally characterize the set of equilibrium selection processes where the gradient with respect to a sampled equilibrium is an unbiased estimate of the true gradient. We evaluate our approach experimentally against existing baselines in three Stackelberg problems with multiple followers and find that in each case, our approach is able to achieve higher utility for the leader.

==> alternative-derivative.tex <==

\subsection{Nikaido–Isoda Function}
\begin{definition}
The Nikaido–Isoda (NI) function introduced by Nikaido et al.~\cite{nikaido1955note} is 
\begin{align}
    \Psi(\boldsymbol\decision, \boldsymbol\otherdecision; \environment) = \sum\nolimits_{i=1}^n f_i(\boldsymbol\decision; \environment) - f_i(\boldsymbol\otherdecision_i, \boldsymbol\decision_{-i}; \environment)
\end{align}
\end{definition}

\begin{definition}
\begin{align}
    V(\boldsymbol\decision; \environment) = \max\nolimits_{\boldsymbol\otherdecision} \Psi(\boldsymbol\decision, \boldsymbol\otherdecision; \environment) \geq 0
\end{align}
\end{definition}

The Nikaido-Isoda function achieves its global minimum $V(\boldsymbol\decision) = 0$ if and only if $\boldsymbol\decision$ is a Nash equilibrium of the game~\eqref{eqn:opt}.
Specifically, we can write down an optimization problem which tries to minimize the Nikaido-Isoda function under feasibility constraints:
\begin{align}
    \min\nolimits_{\boldsymbol\decision} \quad & V(\boldsymbol\decision; \environment) \\
    \text{s.t.} \quad & G_i \decision_i \leq h_i, A_i \decision_i = b_i ~\forall i \in [n]
\end{align}

Interestingly, at the optimality, the solution must also satisfy the KKT conditions:
\begin{align}
    & \nabla_\decision V + G^\top \boldsymbol\lambda + A^\top \boldsymbol\nu = 0 \\
    & D(\boldsymbol\lambda) (G \boldsymbol\decision - \boldsymbol h) = 0 \\
    & A \boldsymbol\decision = \boldsymbol b
\end{align}

Similarly, we can differentiate through the KKT condition and compute $\frac{\partial \boldsymbol\decision}{\partial \environment}$ by:

\begin{align}
    \begin{bmatrix}
    \frac{d \boldsymbol\decision}{d \environment} \\
    \frac{d \boldsymbol\lambda}{d \environment} \\
    \frac{d \boldsymbol\nu}{d \environment}
    \end{bmatrix}
    = 
    \begin{bmatrix}
        \nabla^2_{\boldsymbol\decision} V & G^\top & A^\top \\
        D({\boldsymbol\lambda^*}) G & D(G \boldsymbol\decision^* - h) & 0 \\
        A & 0 & 0
    \end{bmatrix}^{-1}
    \begin{bmatrix}
    \nabla_{\environment \boldsymbol\decision} V \\
    0 \\
    0
    \end{bmatrix}\label{eqn:kkt_derivative_close_form_variant}
\end{align}

Comparing Equation~\eqref{eqn:kkt_derivative_close_form} and~\eqref{eqn:kkt_derivative_close_form_variant}, although the optimization problems being solved by two systems are different, the primal solutions are the same due to the property of the Nikaido-Isoda function and Nash equilibrium.
 That implies the term $\frac{d \boldsymbol\decision}{d \environment}$ in both equations should match.

{\color{red} I don't know how to use this but it is interesting. There are two ways to compute the same $dx/d\pi$ term but one is significantly simpler than the other one.}

==> approximate.tex <==

\section{Approximate KKT Conditions}
It is possible that the solution $\boldsymbol\decision$ is not a Nash equilibrium or even the Nash equilibrium does not exist.
Instead of differentiating through a KKT condition at the optimality, we can differentiate through an approximate KKT condition.
Before dive into differentiating through approximate KKT condition, we first recall the definition of Nikaido–Isoda Function.

\subsection{Nikaido–Isoda Function}
\begin{definition}
The Nikaido–Isoda (NI) function introduced by Nikaido et al.~\cite{nikaido1955note} is 
\begin{align}
    \Psi(\boldsymbol\decision, \boldsymbol\otherdecision; \environment) = \sum\nolimits_{i=1}^n f_i(\boldsymbol\decision; \environment) - f_i(\boldsymbol\otherdecision_i, \boldsymbol\decision_{-i}; \environment)
\end{align}
\end{definition}

\begin{definition}
\begin{align}
    V(\boldsymbol\decision; \environment) = \max\nolimits_{\boldsymbol\otherdecision} \Psi(\boldsymbol\decision, \boldsymbol\otherdecision; \environment) \geq 0
\end{align}
\end{definition}

\begin{theorem}[\citeauthor{krawczyk2000relaxation,uryas1994relaxation}]
When the strategy space is separable, i.e., $\boldsymbol\decisionset = \decisionset_1 \times \decisionset_2 \times \cdots \times \decisionset_n$, $\boldsymbol\decision \in \boldsymbol\decisionset$ is a Nash equilibrium if and only if $V(\boldsymbol\decision; \environment) = 0$.
\end{theorem}
Specifically, we can write down an optimization problem which tries to minimize the Nikaido-Isoda function under feasibility constraints:
\begin{align}
    & \min\nolimits_{\boldsymbol\decision} \quad V(\boldsymbol\decision; \environment) \quad & \text{s.t.} \quad \decision_i \in \decisionset_i  \quad \forall i \in [n]
\end{align}
This optimization problem is able to solve the equilibrium 

\subsection{Approximate KKT Conditions}

We first recall the definition of $\epsilon$-KKT condition mentioned by ~\citeauthor{dutta2013approximate} in the optimization literature. Here we consider optimizing a function $f(\decision)$ subject to constraint $0^m \leq g(\decision) \in \R^m$, which is equivalent to our setting when there is only a single agent.




\begin{definition}
$\decision$ is an $\epsilon$-KKT point of the optimization problem $\min f(\decision) ~\text{s.t.} g(\decision) \leq 0$ if:
\begin{align}
    \norm{\nabla_\decision f(\decision) + \lambda^\top \nabla g(\decision)} \leq \epsilon, \quad \lambda_j g_j(\decision) = 0 ~\forall j \in [m]
\end{align}
\end{definition}
However, as mentioned by \citeauthor{dutta2013approximate}, this definition of $\epsilon$-KKT point is not smooth in $\decision$.
It is possible that the error can increase drastically when we perturb the primal solution $\decision$ a little.
Therefore, \citeauthor{dutta2013approximate} proposed to use the following modified definition:

\begin{definition}
$\boldsymbol\decision$ is a modified $\epsilon$-KKT point of the optimization problem if $~\exists \hat{\decision}$ s.t. $\norm{\hat{\decision} - \decision} \leq \epsilon$ and
\begin{align}
    \norm{\nabla_\decision f(\hat{\decision}) + \boldsymbol\lambda^\top \nabla g(\hat{\decision})} \leq \sqrt{\epsilon}, \quad \boldsymbol\lambda^\top g(\decision) \geq - \epsilon
\end{align}
\end{definition}

\begin{theorem}[\citeauthor{dutta2013approximate}]
If $\decision$ is an $\epsilon$ optimal point of the optimization problem, then $\decision$ is also a modified $\epsilon$-KKT point.
\end{theorem}


In our case, since we have all the agents optimizing their own objectives, it is necessary to take all the agents' KKT conditions into account.
Therefore, we introduce the concept of modified $\epsilon$-KKT point of the multi-agent system as below:

\begin{definition}
$\{ \decision \}_{i \in [n]}$ is a modified $\epsilon$-KKT point of the multi-agent system if there exists $\epsilon_i \geq 0 ~\forall i \in [n]$ with $\sum\nolimits_{i=1}^n \epsilon = \epsilon$ and there exists $\hat{\decision_i}$ with $\norm{\hat{\decision_i} - \decision_i} \leq \epsilon_i ~\forall i \in [n]$ such that:
\begin{align}
    \norm{\nabla_\decision f_i(\hat{\decision_i}, \decision_{-i}) + \lambda_i^\top \nabla g_i(\hat{\decision_i}, \decision_{-i})} \leq \sqrt{\epsilon_i} \\
    \lambda_i^\top g_i(\decision) \geq - \epsilon_i ~\forall i \in [n]
\end{align}
where $\sum\nolimits_{i \in [n]} \epsilon_i \leq \epsilon$.
\end{definition}

{\color{red} TODO}



\begin{theorem}\label{thm:nikaido-isoda-modified-kkt}
Given a feasible solution $\boldsymbol\decision$ with Nikaido-Isoda function value $V(\boldsymbol\decision) \leq \epsilon$, then $\boldsymbol\decision$ is a modified $\epsilon$-KKT point of the multi-agent system.
\end{theorem}
\begin{proof}
We have
\begin{align}
\epsilon \geq V(\boldsymbol\decision) &= \max\nolimits_{\boldsymbol\otherdecision} \Psi(\boldsymbol\decision, \boldsymbol\otherdecision; \environment) \nonumber \\
&= \sum\nolimits_{i=1}^n \max\nolimits_{\otherdecision_i} f_i(\boldsymbol\decision; \environment) - f_i(\boldsymbol\otherdecision_i, \boldsymbol\decision_{-i}; \environment) \nonumber \\
&= \sum\nolimits_{i=1}^n \epsilon_i
\end{align}
where $0 \leq \epsilon_i \coloneqq \max\nolimits_{\otherdecision_i} f_i(\boldsymbol\decision; \environment) - f_i(\boldsymbol\otherdecision_i, \boldsymbol\decision_{-i}; \environment)$.
This implies the solution $\decision_i$ is an $\epsilon_i$ optimal to the $i$-th player's optimization problem.
According to the result from \citeauthor{dutta2013approximate}, $\decision_i$ is a modified $\epsilon_i$-KKT condition to the $i$-th player's optimization problem, i.e. for all $i \in [n]$,
\begin{align}
    \exists \hat{\decision_i}, \lambda_i, \nu_i ~\text{s.t.} & \norm{\decision_i - \hat{\decision_i}} \leq \sqrt{\epsilon_i} \nonumber \\
    & \norm{\nabla f_i(\hat{\decision_i}, \decision_{-i}; \environment) + G_i^\top \lambda_i + A_i^\top \nu_i} \leq \sqrt{\epsilon_i} \nonumber \\
    & \lambda_i^\top (G_i \boldsymbol\decision - h_i) \geq -\epsilon_i
\end{align}
{\color{red} TODO! This is not completely correct unless we change the definition of modified eps-KKT system!?}

We can collect all dual variables and form a meta dual variable $\lambda = [\lambda_1, \lambda_2, \dots, \lambda_n], \nu = [\nu_1, \nu_2, ..., \nu_n]$.
We claim that this meta dual variable yields an error at most $\epsilon$ to the KKT condition of the entire system.

Since each $i$-th coordinate contributes at most error with norm $\sqrt{\epsilon_i}$, the norm of the entire error is given the square root of the sum of all the square term, which is bounded by $\sqrt{\sum\nolimits_{i=1}^n \epsilon_i} = \sqrt{\epsilon}$.
On the other hand, we have $\lambda_i^\top (G_i \boldsymbol\decision - h_i) \geq -\epsilon_i \geq -\epsilon$, which holds for all $i$ unconditionally.
This concludes the proof that the meta dual variables $\lambda, \nu$ yield a KKT condition with modified error at most $\epsilon$, thus also a modified $\epsilon$-KKT condition.
\end{proof}

\subsection{Convergence of Modified $\epsilon$-KKT Points}
\begin{theorem}
If we have a series of points $\boldsymbol\decision^j$ where $\boldsymbol\decision^j$ is a modified $\epsilon^j$-KKT point of the multi-agent system and $\lim\nolimits_{j \rightarrow \infty} \boldsymbol\decision^j = \boldsymbol\decision$ and $\lim\nolimits_{j \rightarrow \infty} \epsilon^j = \epsilon$, then $\boldsymbol\decision$ is a modified $\epsilon$-KKT point of the multi-agent system.
\end{theorem}
\begin{proof}
{\color{red} TODO! Have not figured out how to prove this but it looks correct to me.}
\end{proof}


\subsection{Approximate Nash Equilibrium}
In the above analysis, we require to compute a Nash equilibrium.
However, it is often hard to compute in many games.
Oftentimes, we are only able to achieve an $\epsilon$-Nash equilibrium.
Here, we characterize the impact to the KKT conditions of each agent and then provide a regularization based approach to resolve the issue of back-propagating through the KKT conditions with approximate solution.

We first recall the definition of $\epsilon$-Nash equilibrium.

\begin{definition}
$\{ \decision^*_i \}_{i \in [n]}$ is called $\epsilon$-Nash equilibrium if
\begin{align}
    f_i(\decision_i, \decision_{-i}) \geq \max\nolimits_{y_i \in \decisionset_i} f_i(y_i, \decision_{-i}) - \epsilon \quad\quad \forall i \in [n]
\end{align}
\end{definition}


\begin{proposition}
$\boldsymbol\decision$ is $\frac{\epsilon}{n}$-Nash $\Rightarrow$ $\boldsymbol\decision$ is an $\epsilon$-optimum of Nikaido-Isoda function $\Rightarrow$ $\boldsymbol\decision$ is a modified $\epsilon$-KKT point
\end{proposition}
\begin{proof}
The first part of the proof is due to:
\begin{align*}
    V(\boldsymbol\decision) & = \max\nolimits_{\boldsymbol y} \Psi(\boldsymbol\decision, \boldsymbol y; \environment) \\
    & = \sum\nolimits_{i=1}^n \max\nolimits_{y_i \in \decisionset_i} f_i(\boldsymbol\decision; \environment) - f_i(y_i, \decision_{-i}; \environment) \leq n \cdot \frac{\epsilon}{n} = \epsilon
\end{align*}
The second part of the proof directly follows by Theorem~\ref{thm:nikaido-isoda-modified-kkt}.
\end{proof}


\subsection{Conservation Law of Approximate Equilibria}

%\subsection{Sequential Games}
%Let us use a two-player Stackelberg game to illustrate the differentiability idea in sequential games.
%Let the leader to be player 0 and the follower to be player 1.
%Our historical dataset contains data with $a_0, a_1$, where player 1 is fully rational and plays optimally.
%This games needs not be zero-sum, which can still be written as a bilevel optimization problem.
%We assume the leader does not know the follower's payoff value (private information) and it has to be inferred from the historical plays.

%Thus, one can try to minimize the mismatch between the predicted player 1's action and the historical action:
%\begin{align}
%    & \min\limits_{\theta} \frac{1}{m} \sum\nolimits_{j \in [m]} || a_1^j - \hat{a}_1^j|| \\
%    \text{s.t.} \quad & \hat{a}_1^j \in \arg\max\nolimits_{\hat{a}_1^j \in A_1} f_1(a_0^j, \hat{a}_1^j, \theta) ~\forall j \in [m]
%\end{align}
%Given the optimality of player 1, we know that the KKT conditions of player 1's decision must hold.
%\begin{align}
%    \nabla_{a_1} f_1(a_0^j, \hat{a}_1^j, \theta) + \lambda^j \nabla_{a_1} g_1(\hat{a}_1^j) = 0 \\
%    g_1(\hat{a}_1^j) \leq 0 \\
%    \lambda^j \geq 0
%\end{align}

%We can differentiate through the KKT conditions to obtain the derivative of $\theta$:
%\begin{align}
%    \frac{\partial}{\partial \theta} KKT = 0 \Rightarrow \frac{\partial \hat{a}_1^j}{\partial \theta} = ...
%\end{align}

==> backup.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{figures/qre/qre-unconstrained-obj.pdf}
        \caption{Quantal response equilibrium}
        \centering
        \label{fig:QRE-quality}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{figures/ssg/ssg-unconstrained-obj.pdf}
        \caption{Uncoordinated defenders in SSGs}
        \label{fig:ssg-quality}
        \centering
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{example-image-c}
        \caption{Cyber insurance games}
        \label{fig:cyber-insurance}
        \centering
    \end{subfigure}
    \caption{When the constraints are independent on the resulted equilibrium, we apply Algorithm~\ref{alg:differentiable-equilibrium} to compute the derivative and run projected gradient descent to find the optimal policy with maximum expected social welfare at equilibrium.}
    \label{fig:quality}
\end{figure*}
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{figures/qre/qre-constrained-obj.pdf}
        \caption{Quantal response equilibrium}
        \centering
        \label{fig:qre-unconstrained-obj}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{figures/ssg/ssg-constrained-obj.pdf}
        \caption{Uncoordinated defenders in SSGs}
        \label{fig:ssg-quality-constrained}
        \centering
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \includegraphics[width=\textwidth]{figures/cyber/cyber-constrained-obj.pdf}
        \caption{Cyber insurance games}
        \label{fig:cyber-insurance-constrained}
        \centering
    \end{subfigure}
    \caption{When the constraints are dependent on the resulted equilibrium, we apply Algorithm~\ref{alg:constrained-differentiable-equilibrium} to compute the derivative and run augmented Lagrangian method to find the optimal policy with maximum expected social welfare and minimum constraint violation at equilibrium.}
    \label{fig:quality-constrained}
\end{figure*}

==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{The algorithm on multiple equilibria relies on Theorem~\ref{thm:sufficient-conditions} to hold as we discuss in Section~\ref{sec:multiple-equilibria}. Please refer to Section~\ref{sec:multiple-equilibria} and Appendix~\ref{sec:limitations} for more detailed discussion.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Proof sketches are provided in the main paper and the full proofs can be found in Appendix~\ref{sec:missing-proofs}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please refer to the supplemental material for code.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to Appendix~\ref{sec:experimental-setup} for experimental setup.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to Appendix~\ref{sec:computing-infrastructure}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
